Gender Bias in Explainability: Investigating Performance Disparity in Post-hoc Methods

While research on applications and evaluations of explanation methods continues to expand, fairness of the explanation methods concerning disparities in their performance across subgroups remains an often overlooked aspect. In this paper, we address this gap by showing that, across three tasks and five language models, widely used post-hoc feature attribution methods exhibit significant gender disparity with respect to their faithfulness, robustness, and complexity. These disparities persist even when the models are pre-trained or fine-tuned on particularly unbiased datasets, indicating that the disparities we observe are not merely consequences of biased training data. Our results highlight the importance of addressing disparities in explanations when developing and applying explainability methods, as these can lead to biased outcomes against certain subgroups, with particularly critical implications in high-stakes contexts. Furthermore, our findings underscore the importance of incorporating the fairness of explanations, alongside overall model fairness and explainability, as a requirement in regulatory frameworks.

==> figures/heatmap.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/heatmap.pdf}
    \caption{Heatmap of how many repeats out of 5 shows significant bias ($p \leq 0.05$) and towards which gender, after 50 epochs of fine-tuning. Blue indicates males have higher scores and reds females. (Cmp: Comprehensiveness (AOPC) ($\uparrow$), Gini: Gini index ($\uparrow$) Loo: Correlation with LOO scores ($\uparrow$), MAc: Mass accuracy ($\uparrow$), Sff: Sufficiency (AOPC) ($\downarrow$), Spr: Sparsity ($\downarrow$))}
    \label{fig:heatmap}
\end{figure*}

==> tables/OLD_full_table.tex <==
\begin{table*}[h!]
    \caption{How many repeats out of 5 shows significant bias (indicated in parenthesis) and average effect sizes (Cohen's $d$), $\pm$ standard deviations, after 50 epochs of fine-tuning. \textbf{Bold} indicates considerable effect size (absolute value $\geq 0.2$). $N_{\text{disp.}}, N_{\text{disp.}}^*$ indicate per row the number of significant disparities and those with an absolute effect size of at least $0.2$.}
    \label{tab:main_results}
    \centering
    \tiny
    \begin{tabular}{lllllllllrr}
        \toprule
        \textbf{Dataset} & \textbf{Model} & \textbf{Method} & AOPC Comp. ($\uparrow$) & Corr. LOO ($\uparrow$) & Mass Acc. ($\uparrow$) & AOPC Suff. ($\downarrow$) & Gini Index ($\uparrow$) & Sparsity ($\downarrow$) & $N_{\text{disp.}}$ & $N_{\text{disp.}}^*$ \\
        \midrule
        \multirow[t]{24}{*}{ALL} & \multirow[t]{6}{*}{BERT} & Grad & \textbf{(3) -.81±2.62} & (0) NA & (5) .12±.41 & \textbf{(5) -.24±.15} & (4) .03±.60 & (3) .08±.17 & 20/30 & 8/30 \\
         &  & GxI & (1) -.05±.00 & (0) NA & (2) .10±.00 & (2) .01±.88 & (2) .05±.38 & (0) NA & 7/30 & 0/30 \\
         &  & IG & (2) .11±.48 & (0) NA & (2) -.08±.00 & \textbf{(1) -.83±.00} & (4) -.15±.37 & (0) NA & 9/30 & 1/30 \\
         &  & IGxI & \textbf{(2) -.28±1.17} & (0) NA & \textbf{(3) -.47±.23} & (4) -.11±.10 & \textbf{(5) -.27±.91} & \textbf{(4) .38±.15} & 18/30 & 14/30 \\
         &  & LIME & \textbf{(5) -.52±1.20} & (0) NA & \textbf{(1) .51±.00} & (3) .08±.13 & \textbf{(5) -.57±1.10} & (3) -.09±.13 & 17/30 & 11/30 \\
         &  & SHAP & \textbf{(4) -.44±1.36} & (0) NA & \textbf{(3) .30±.22} & (3) .15±.28 & \textbf{(3) -.28±1.01} & \textbf{(1) -.35±.00} & 14/30 & 11/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{FairBERTa} & Grad & \textbf{(5) -1.64±1.13} & (0) NA & (4) .18±.02 & \textbf{(5) -.25±.09} & \textbf{(2) .27±.41} & (1) .19±.00 & 17/30 & 12/30 \\
         &  & GxI & \textbf{(4) -.37±.17} & (0) NA & (1) -.05±.00 & \textbf{(4) -.58±.56} & \textbf{(1) -.22±.00} & (0) NA & 10/30 & 9/30 \\
         &  & IG & \textbf{(4) -.30±.15} & (0) NA & (0) NA & \textbf{(2) -.75±.05} & \textbf{(4) -.32±.12} & (1) .15±.00 & 11/30 & 10/30 \\
         &  & IGxI & \textbf{(5) -1.00±.47} & (0) NA & (3) .15±.06 & (5) -.06±.05 & \textbf{(5) -.85±.47} & \textbf{(4) .34±.17} & 22/30 & 14/30 \\
         &  & LIME & \textbf{(5) -1.63±.65} & (0) NA & (4) .05±.13 & (4) -.04±.04 & \textbf{(4) -.94±.58} & \textbf{(2) .22±.05} & 19/30 & 11/30 \\
         &  & SHAP & \textbf{(5) -1.64±.63} & (0) NA & \textbf{(5) .21±.15} & (4) -.06±.04 & \textbf{(4) -1.06±.62} & \textbf{(2) .26±.06} & 20/30 & 16/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{GPT2} & Grad & \textbf{(5) .34±1.53} & (0) NA & (4) .07±.27 & \textbf{(5) .28±.71} & \textbf{(3) -.23±.29} & (0) NA & 17/30 & 13/30 \\
         &  & GxI & (4) -.18±.15 & (0) NA & (3) -.09±.09 & \textbf{(4) .24±1.01} & (5) -.03±.44 & (1) .16±.00 & 17/30 & 4/30 \\
         &  & IG & \textbf{(3) -.38±.15} & (0) NA & (0) NA & (4) .20±.67 & \textbf{(3) -.25±.47} & (2) .16±.02 & 12/30 & 6/30 \\
         &  & IGxI & \textbf{(4) -.96±.81} & (0) NA & \textbf{(1) -.63±.00} & \textbf{(3) .34±.74} & \textbf{(4) -.54±1.68} & (5) .17±.27 & 17/30 & 12/30 \\
         &  & LIME & \textbf{(4) -.89±.29} & (0) NA & (4) -.02±.09 & \textbf{(5) .34±.57} & \textbf{(5) .41±.45} & (0) NA & 18/30 & 14/30 \\
         &  & SHAP & \textbf{(5) -1.33±.67} & (0) NA & \textbf{(5) .37±.34} & \textbf{(3) .25±.65} & \textbf{(2) -.62±1.02} & (3) .16±.07 & 18/30 & 15/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{TinyBERT} & Grad & \textbf{(5) -.33±.88} & (0) NA & \textbf{(5) .46±.21} & (4) .02±.09 & (5) -.12±.62 & (1) .10±.00 & 20/30 & 10/30 \\
         &  & GxI & \textbf{(5) -.60±.60} & \textbf{(2) .21±.05} & (5) .05±.08 & \textbf{(5) .22±.47} & \textbf{(4) -.73±.60} & \textbf{(3) .23±.08} & 24/30 & 19/30 \\
         &  & IG & (3) -.17±.44 & \textbf{(1) .27±.00} & (3) -.00±.10 & (2) .05±.34 & (4) .03±.70 & (1) .07±.00 & 14/30 & 1/30 \\
         &  & IGxI & \textbf{(5) -.37±.39} & \textbf{(2) -.58±.02} & \textbf{(5) -.26±.35} & (3) -.00±.06 & \textbf{(5) -1.44±1.36} & \textbf{(2) .34±.02} & 20/30 & 19/30 \\
         &  & LIME & \textbf{(5) -.60±.52} & \textbf{(1) -.40±.00} & (2) -.02±.12 & (5) .05±.04 & \textbf{(5) -1.01±.61} & (2) -.08±.20 & 20/30 & 11/30 \\
         &  & SHAP & \textbf{(4) -.79±.28} & \textbf{(2) -.76±.08} & (3) -.11±.15 & (3) .06±.07 & \textbf{(5) -.97±1.62} & (1) -.18±.00 & 18/30 & 11/30 \\
        \midrule
        \multirow[t]{24}{*}{SUBJ} & \multirow[t]{6}{*}{BERT} & Grad & \textbf{(5) .35±.65} & (0) NA & \textbf{(1) .22±.00} & (4) .05±.32 & (3) .05±.33 & (2) .07±.09 & 15/30 & 6/30 \\
         &  & GxI & (3) .15±.29 & \textbf{(1) -.21±.00} & (0) NA & (4) .04±.44 & (2) -.05±.20 & (0) NA & 10/30 & 1/30 \\
         &  & IG & \textbf{(2) .22±.00} & (1) .18±.00 & (1) .02±.00 & (4) .11±.36 & (4) -.10±.55 & \textbf{(1) .37±.00} & 15/30 & 3/30 \\
         &  & IGxI & (3) -.01±.48 & \textbf{(1) .21±.00} & (5) -.05±.15 & (4) .10±.12 & \textbf{(4) -.51±.61} & \textbf{(2) .28±.11} & 19/30 & 7/30 \\
         &  & LIME & (4) .19±.48 & \textbf{(1) .22±.00} & (3) -.13±.22 & (5) .10±.05 & \textbf{(4) -.54±.36} & \textbf{(2) .34±.20} & 19/30 & 7/30 \\
         &  & SHAP & (3) .12±.56 & \textbf{(1) -.44±.00} & \textbf{(3) -.53±.22} & (4) .13±.08 & \textbf{(4) -.67±.67} & \textbf{(4) .22±.28} & 19/30 & 12/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{FairBERTa} & Grad & \textbf{(4) -.37±.17} & (5) .07±.33 & (3) .19±.05 & (3) -.16±.18 & (5) .18±.35 & (1) .14±.00 & 18/30 & 4/30 \\
         &  & GxI & \textbf{(3) -.28±.13} & \textbf{(1) -.27±.00} & (1) .07±.00 & (4) -.11±.27 & \textbf{(2) .21±.01} & (0) NA & 11/30 & 6/30 \\
         &  & IG & (1) .10±.00 & (0) NA & (0) NA & \textbf{(1) -.57±.00} & \textbf{(1) -.27±.00} & (0) NA & 3/30 & 2/30 \\
         &  & IGxI & \textbf{(5) -.48±.15} & (3) .06±.33 & \textbf{(1) .38±.00} & (4) .04±.10 & \textbf{(5) -.47±.18} & (3) .20±.01 & 21/30 & 11/30 \\
         &  & LIME & \textbf{(5) -.56±.24} & (3) -.09±.38 & (3) -.03±.14 & (3) -.08±.13 & \textbf{(4) -.47±.20} & \textbf{(4) .23±.17} & 22/30 & 13/30 \\
         &  & SHAP & \textbf{(5) -.48±.22} & (3) -.01±.32 & (5) .12±.03 & (4) -.04±.14 & (1) -.16±.00 & (1) .14±.00 & 19/30 & 5/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{GPT2} & Grad & \textbf{(4) -.53±.73} & \textbf{(1) .26±.00} & (3) .19±.33 & (5) .11±.45 & \textbf{(3) .25±.34} & (0) NA & 16/30 & 8/30 \\
         &  & GxI & \textbf{(3) -.59±.29} & (0) NA & (3) -.00±.19 & (5) -.10±.44 & (4) .18±.28 & (2) -.17±.00 & 17/30 & 3/30 \\
         &  & IG & \textbf{(4) -.46±.20} & (0) NA & (2) -.04±.02 & \textbf{(3) -.30±.53} & \textbf{(5) -.38±.39} & (0) NA & 14/30 & 12/30 \\
         &  & IGxI & \textbf{(4) -1.12±.27} & (0) NA & (3) -.12±.14 & (5) .11±.19 & \textbf{(4) -.87±.32} & \textbf{(2) .29±.09} & 18/30 & 10/30 \\
         &  & LIME & \textbf{(5) -.86±.18} & \textbf{(1) 1.06±.00} & (5) -.07±.13 & (5) .05±.27 & (4) .11±.50 & (0) NA & 20/30 & 6/30 \\
         &  & SHAP & \textbf{(5) -1.12±.22} & \textbf{(1) 1.39±.00} & \textbf{(5) -.21±.79} & (4) .02±.31 & (4) -.16±.44 & \textbf{(1) .21±.00} & 20/30 & 12/30 \\
        \cmidrule{2-11}
         & \multirow[t]{6}{*}{TinyBERT} & Grad & \textbf{(5) -.71±1.09} & (3) -.10±.22 & \textbf{(2) .56±.06} & (5) -.08±.10 & \textbf{(3) -.31±.13} & (2) .18±.07 & 20/30 & 10/30 \\
         &  & GxI & \textbf{(4) -.74±.08} & \textbf{(4) -.32±.29} & (5) .01±.08 & \textbf{(5) .24±.62} & \textbf{(4) -.73±.39} & \textbf{(2) .33±.10} & 24/30 & 19/30 \\
         &  & IG & (5) -.11±.27 & \textbf{(2) .29±.51} & (2) .18±.09 & \textbf{(4) -.57±.67} & (4) -.19±.35 & (1) .14±.00 & 18/30 & 6/30 \\
         &  & IGxI & \textbf{(5) -.55±.34} & (4) -.04±.40 & \textbf{(5) -.33±.37} & (4) .02±.09 & \textbf{(4) -1.60±1.14} & \textbf{(3) .55±.07} & 25/30 & 17/30 \\
         &  & LIME & \textbf{(5) -.67±.43} & \textbf{(3) -.29±.11} & (2) .02±.09 & (2) .05±.01 & \textbf{(5) -1.39±.37} & \textbf{(4) .39±.13} & 21/30 & 17/30 \\
         &  & SHAP & \textbf{(5) -.71±.44} & (4) -.19±.31 & \textbf{(2) .40±.26} & (2) .10±.07 & \textbf{(4) -1.44±.32} & \textbf{(5) .39±.29} & 22/30 & 16/30 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/compas_table.tex <==
\begin{table}
\centering
\caption{\label{tab:compas}\textbf{COMPAS}. Counts of significant disparity with colors indicating direction of effect (red=negative, blue=positive)}
\small
\begin{tabular}{clrrrrrrr}
    \toprule
    & & 
    \multicolumn{7}{c}{COMPAS} \\
    \cmidrule{3-9}
    \textbf{Model} & \textbf{Method} & \rot{90}{Compr.} & \rot{90}{Suff.} & \rot{90}{Soft Compr.} & \rot{90}{Soft Suff.} & \rot{90}{Gini} & \rot{90}{Spars.} & \rot{90}{Sens.}  \\
    \midrule
     &  Grad &  \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!20.0}2} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
    &  IG &  \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!50.0}5} \\
     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{TinyBERT}}} &  IGxI &  \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} \\
    &  LIME &  {\cellcolor{blue!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!30.0}3} \\
    &  SHAP &  \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} \\
    \cmidrule{1-9}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} & {\cellcolor{red!40.0}4} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} \\
    &  IG &  {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{GPT2}}} &  IGxI &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!10.0}1} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} \\
    &  SHAP &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!30.0}3} & 0 & 0 & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} \\
    \cmidrule{1-9}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!20.0}2} \\
    &  IG &  \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!30.0}3} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{BERT}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!30.0}3} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!30.0}3} \\
    &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} \\
    \cmidrule{1-9}
     &  Grad &  \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!40.0}4} & 0 & {\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!20.0}2} & {\cellcolor{blue!30.0}3} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{red!30.0}3} & {\cellcolor{blue!40.0}4} \\
    &  IG &  {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!40.0}4} & {\cellcolor{blue!20.0}2} & {\cellcolor{red!20.0}2} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{FairBERTa}}} &  IGxI &  {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!10.0}1} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!30.0}3} \\
    &  LIME &  \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!30.0}3} \\
    &  SHAP &  \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!10.0}1} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!20.0}2} & {\cellcolor{blue!40.0}4} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!30.0}3} \\
    \cmidrule{1-9}
     &  Grad &  {\cellcolor{blue!30.0}3} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!20.0}2} & {\cellcolor{red!30.0}3} & 0 & 0 \\
    &  GxI &  {\cellcolor{blue!10.0}1} & {\cellcolor{red!20.0}2} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!10.0}1} & 0 \\
    &  IG &  \textbf{\cellcolor{red!10.0}1} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!10.0}1} & 0 \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{RoBERTa}}} &  IGxI &  {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!10.0}1} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!30.0}3} & 0 \\
    &  LIME &  \textbf{\cellcolor{red!10.0}1} & {\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & {\cellcolor{red!10.0}1} & 0 & 0 \\
    &  SHAP &  {\cellcolor{blue!20.0}2} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!20.0}2} & {\cellcolor{red!40.0}4} & 0 \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/counts_table.tex <==
% \begin{table}
% \centering
% \caption{\label{tab:new_all_table}\textbf{Number of runs out of five resulting in statistically significant disparity} on the GECO datasets. Colors of the cells indicate which gender has higher evaluation scores (blue: males, red: females). Bold font further indicates considerable effect size (Cohen's $d$, with $\vert d \vert \geq 0.2$).}
% \small
% \begin{tabular}{clrrrrrrr|rrrrrrr}
%     \toprule
%     & & 
%     \multicolumn{7}{c|}{GECO-ALL} & \multicolumn{7}{c}{GECO-SUBJ} \\
%     \cmidrule{3-16}
%     \textbf{Model} & \textbf{Method} & \rot{90}{Compr.} & \rot{90}{Suff.} & \rot{90}{Soft Compr.} & \rot{90}{Soft Suff.} & \rot{90}{Gini} & \rot{90}{Spars.} & \rot{90}{Sens.} & \rot{90}{Compr.} & \rot{90}{Suff.} & \rot{90}{Soft Compr.} & \rot{90}{Soft Suff.} & \rot{90}{Gini} & \rot{90}{Spars.} & \rot{90}{Sens.} \\
%     \midrule
%      &  Grad &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!30.0}3} & 0 & \textbf{\cellcolor{red!40.0}4} \\
%     &  GxI &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!30.0}3} & 0 & \textbf{\cellcolor{red!40.0}4} \\
%     &  IG &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!40.0}4} \\
%     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{TinyBERT}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
%     &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
%     &  SHAP &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
%     \cmidrule{1-16}
%      &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} \\
%     &  GxI &  {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!50.0}5} \\
%     &  IG &  \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!10.0}1} & 0 & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!10.0}1} & 0 & {\cellcolor{blue!50.0}5} \\
%     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{GPT2}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{blue!50.0}5} \\
%     &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!40.0}4} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} \\
%     &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} \\
%     \cmidrule{1-16}
%      &  Grad &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & \textbf{\cellcolor{blue!40.0}4} \\
%     &  GxI &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{blue!30.0}3} \\
%     &  IG &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!30.0}3} & 0 & \textbf{\cellcolor{blue!40.0}4} \\
%     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{BERT}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & \textbf{\cellcolor{blue!30.0}3} \\
%     &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!40.0}4} \\
%     &  SHAP &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!40.0}4} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!40.0}4} \\
%     \cmidrule{1-16}
%      &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{blue!40.0}4} \\
%     &  GxI &  \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & 0 & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & {\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!40.0}4} \\
%     &  IG &  \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!20.0}2} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{blue!40.0}4} \\
%     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{FairBERTa}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!40.0}4} \\
%     &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!40.0}4} \\
%     &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!40.0}4} \\
%     \cmidrule{1-16}
%      &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & 0 & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & 0 & \textbf{\cellcolor{blue!50.0}5} \\
%     &  GxI &  \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & 0 & \textbf{\cellcolor{blue!50.0}5} \\
%     &  IG &  {\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & 0 & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & 0 & \textbf{\cellcolor{blue!50.0}5} \\
%     \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{RoBERTa}}} &  IGxI &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!10.0}1} & 0 & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!20.0}2} & {\cellcolor{blue!20.0}2} & \textbf{\cellcolor{blue!50.0}5} \\
%     &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} \\
%     &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{blue!50.0}5} \\
%     \bottomrule
% \end{tabular}
% \end{table}

\begin{table*}
\centering
\caption{\label{tab:new_all_table}\textbf{Number of runs out of five resulting in statistically significant disparity} on the GECO datasets. Cell colors indicate which gender has better evaluation scores for each metric (blue: males, red: females). Bold font further indicates considerable effect size (Cohen's $d$, with $\vert d \vert \geq 0.2$).}
\small
\begin{tabular}{clrrrrrrr|rrrrrrr}
    \toprule
    & & 
    \multicolumn{7}{c|}{GECO-ALL} & \multicolumn{7}{c}{GECO-SUBJ} \\
    \cmidrule{3-16}
    \textbf{Model} & \textbf{Method} & \rot{90}{Compr. (F)} & \rot{90}{Suff. (F)} & \rot{90}{Soft Compr. (F)} & \rot{90}{Soft Suff. (F)} & \rot{90}{Gini (C)} & \rot{90}{Spars. (C)} & \rot{90}{Sens. (R)} & \rot{90}{Compr. (F)} & \rot{90}{Suff. (F)} & \rot{90}{Soft Compr. (F)} & \rot{90}{Soft Suff. (F)} & \rot{90}{Gini (C)} & \rot{90}{Spars. (C)} & \rot{90}{Sens. (R)} \\
    \midrule
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{blue!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & 0 & \textbf{\cellcolor{blue!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & 0 & \textbf{\cellcolor{blue!40.0}4} \\
    &  IG &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{TinyBERT}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} \\
    &  SHAP &  \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} \\
    \cmidrule{1-16}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!50.0}5} \\
    &  GxI &  {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} \\
    &  IG &  \textbf{\cellcolor{blue!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!10.0}1} & 0 & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!10.0}1} & 0 & {\cellcolor{red!50.0}5} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{GPT2}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!50.0}5} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!50.0}5} \\
    &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} \\
    \cmidrule{1-16}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & 0 & \textbf{\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{red!30.0}3} \\
    &  IG &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!10.0}1} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!30.0}3} & 0 & \textbf{\cellcolor{red!40.0}4} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{BERT}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & \textbf{\cellcolor{red!30.0}3} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} \\
    &  SHAP &  \textbf{\cellcolor{red!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} \\
    \cmidrule{1-16}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & {\cellcolor{blue!40.0}4} & 0 & \textbf{\cellcolor{red!40.0}4} \\
    &  GxI &  \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!20.0}2} & 0 & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & {\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & {\cellcolor{red!30.0}3} & {\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!40.0}4} \\
    &  IG &  \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!20.0}2} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!40.0}4} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{FairBERTa}}} &  IGxI &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & {\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!30.0}3} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} \\
    &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!40.0}4} & {\cellcolor{blue!50.0}5} & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{red!40.0}4} \\
    \cmidrule{1-16}
     &  Grad &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & 0 & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & 0 & \textbf{\cellcolor{red!50.0}5} \\
    &  GxI &  \textbf{\cellcolor{red!20.0}2} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!20.0}2} & {\cellcolor{red!10.0}1} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & 0 & \textbf{\cellcolor{red!50.0}5} \\
    &  IG &  {\cellcolor{red!30.0}3} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & 0 & {\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!10.0}1} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & 0 & 0 & \textbf{\cellcolor{red!50.0}5} \\
    \multirow[t]{6}{*}{\rotatebox[origin=c]{45}{\textbf{RoBERTa}}} &  IGxI &  \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!10.0}1} & 0 & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & {\cellcolor{red!20.0}2} & {\cellcolor{red!20.0}2} & \textbf{\cellcolor{red!50.0}5} \\
    &  LIME &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} \\
    &  SHAP &  \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{blue!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!50.0}5} & \textbf{\cellcolor{red!40.0}4} & \textbf{\cellcolor{red!50.0}5} \\
    \bottomrule
\end{tabular}
\end{table*}

==> tables/sensitivity_results.tex <==
\begin{table*}[]
    \small
    \centering
    \caption{Preliminary results evaluating the explanations with the sensitivity metric. Numbers in the parentheses indicate how many of the total runs shows significant bias, with average effect sizes (Cohen's $d$) $\pm$ standard deviations after 50 epochs of fine-tuning. \textbf{Bold} indicates considerable effect size (absolute value $\geq 0.2$).}
    \label{tab:sensitivity}
    \begin{tabular}{llllll}
    \toprule
    \textbf{Dataset} & \textbf{Explainer} & \textbf{BERT} & \textbf{FairBERTa} & \textbf{GPT2} & \textbf{TinyBERT} \\
    \midrule
    \multirow[t]{6}{*}{ALL} & Grad & \textbf{(1/1) 1.31±.00} & \textbf{(2/2) .52±.83} & \textbf{(1/1) -2.78±.00} & \textbf{(1/1) 1.67±.00} \\
     & GxI & \textbf{(1/1) 1.34±.00} & \textbf{(2/2) .55±.84} & \textbf{(1/1) -2.33±.00} & \textbf{(1/1) 1.68±.00} \\
     & IG & \textbf{(1/1) 1.33±.00} & \textbf{(2/2) .52±.89} & \textbf{(1/1) -2.64±.00} & \textbf{(1/1) 1.69±.00} \\
     & IGxI & \textbf{(1/1) 1.38±.00} & \textbf{(2/2) .53±.86} & \textbf{(1/1) -1.95±.00} & \textbf{(1/1) 1.66±.00} \\
     & LIME & \textbf{(1/1) 1.35±.00} & \textbf{(2/2) .52±.88} & \textbf{(1/1) -2.64±.00} & \textbf{(1/1) 1.62±.00} \\
     & SHAP & \textbf{(1/1) 1.39±.00} & \textbf{(2/2) .50±.87} & \textbf{(1/1) -2.06±.00} & \textbf{(1/1) 1.77±.00} \\
    \midrule
    \multirow[t]{6}{*}{SUBJ} & Grad & \textbf{(1/1) -.40±.00} & \textbf{(1/1) 1.40±.00} & \textbf{(1/1) -2.93±.00} & \textbf{(1/1) 1.04±.00} \\
     & GxI & \textbf{(1/1) -.33±.00} & \textbf{(1/1) 1.06±.00} & \textbf{(1/1) -1.99±.00} & \textbf{(1/1) 1.07±.00} \\
     & IG & \textbf{(1/1) -.36±.00} & \textbf{(1/1) 1.28±.00} & \textbf{(1/1) -2.12±.00} & \textbf{(1/1) 1.05±.00} \\
     & IGxI & \textbf{(1/1) -.33±.00} & \textbf{(1/1) 1.09±.00} & \textbf{(1/1) -1.61±.00} & \textbf{(1/1) 1.09±.00} \\
     & LIME & \textbf{(1/1) -.40±.00} & \textbf{(1/1) 1.12±.00} & \textbf{(1/1) -2.59±.00} & \textbf{(1/1) 1.01±.00} \\
     & SHAP & \textbf{(1/1) -.34±.00} & \textbf{(1/1) 1.16±.00} & \textbf{(1/1) -1.98±.00} & \textbf{(1/1) 1.05±.00} \\
    \bottomrule
    \end{tabular}
\end{table*}
